Semantic Robustness of Models of Source Code

Deep neural networks are vulnerable to adversarial examples - small input perturbations that result in incorrect predictions. We study this problem for models of source code, where we want the network to be robust to source-code modifications that preserve code functionality. (1) We define a powerful adversary that can employ sequences of parametric, semantics-preserving program transformations; (2) we show how to perform adversarial training to learn models robust to such adversaries; (3) we conduct an evaluation on different languages and architectures, demonstrating significant quantitative gains in robustness.

==> figures/ig-input-classes.tex <==
\newcommand{\up}[1]{\textcolor{PineGreen}{\UParrow}~\textcolor{PineGreen}{#1}}
\newcommand{\down}[1]{\textcolor{Maroon}{\DOWNarrow}~\textcolor{Maroon}{#1}}

\begin{table}[t!]
\center
\small
\caption{
Input token classes in descending order of average IG, for the normally and adversarially trained models on the c2s/java-small dataset (Avg. IG $\times$ 100 in brackets). \textcolor{PineGreen}{Increased} (\textcolor{PineGreen}{\UParrow}) and \textcolor{Maroon}{decreased} (\textcolor{Maroon}{\DOWNarrow}) average IG shown in colors. 
\aws{we've discussed this last time, but wouldn't it make more sense to take absolute IG scores}
}
\label{table:input_classes}
\begin{tabular}{lll}
\toprule
 Normal         & 
 Random-Retarget &   
 Gradient-Retarget 
\\
\midrule
\sc Keyword (2.79) & 
\sc \up{Keyword (3.06)} &
\sc \up{Keyword (3.52)} 
\\
\sc Operator (0.79) & 
\sc \up{Other (0.72)} &  
\sc \up{Operator (1.22)}   
\\
\sc Delimiter (0.71)   & 
\sc \down{Operator (0.71)} &
\sc \down{Delimiter (0.6)} 
\\
\sc Other (0.59)   & 
\sc \down{Delimiter (0.6)} &
\sc \down{Other (0.49)} 
\\
\sc Number (0.02)   & 
\sc \down{Number (-0.16)} &
\sc \up{Number (0.3)} 
\\
\bottomrule
\end{tabular}
\end{table}







==> figures/transforms-table.tex <==
\begin{table}[t]
\caption{
Our suite of semantics-preserving transformations, along with effects of random ($\testRandDepthOne{}$) and gradient-based ($\testGradDepthOne{}$) adversaries \emph{per transformation}, on normally trained models, for the c2s/java-small dataset. 
% \textbf{ Transformations with a comparison of Random (R) vs. Targeted (T) attack strength.}
}
\label{table:transformations}
\centering
% \scriptsize
\scriptsize
\begin{tabular}{lcccc}
\toprule
\multirow{3}{*}{Transform} & \multicolumn{2}{c}{seq2seq (F1: 37.8)} &  \multicolumn{2}{c}{code2seq (F1: 41.4)} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} 
& $\Delta$F1 ($\testRandDepthOne{}$) & $\Delta$F1 ($\testGradDepthOne{}$) &$\Delta$F1 ($\testRandDepthOne{}$) & $\Delta$F1 ($\testGradDepthOne{}$) \\
%  & F1 Drop (R) & F1 Drop (T) & F1 Drop (R) & F1 Drop (T) \\
\midrule
\csvreader[
head to column names,
late after line=\\,
late after last line=\\
]{data/individual-attacks.csv}{}%
{%
\texttt{\attackName} & 
-\randTargFOneDrop &
-\gradTargFOneDrop &
-\randTargFOneDropCS &
-\gradTargFOneDropCS
}%
\end{tabular}
\end{table}
